Bias-Aware Sketches

Linear sketching algorithms have been widely used for processing large-scale distributed and streaming datasets. Their popularity is largely due to the fact that linear sketches can be naturally composed in the distributed model and be efficiently updated in the streaming model. The errors of linear sketches are typically expressed in terms of the sum of coordinates of the input vector excluding those largest ones, or, the mass on the tail of the vector. Thus, the precondition for these algorithms to perform well is that the mass on the tail is small, which is, however, not always the case -- in many real-world datasets the coordinates of the input vector have a {\em bias}, which will generate a large mass on the tail. In this paper we propose linear sketches that are {\em bias-aware}. We rigorously prove that they achieve strictly better error guarantees than the corresponding existing sketches, and demonstrate their practicality and superiority via an extensive experimental evaluation on both real and synthetic datasets.

==> application.tex <==
\section{Applications}
\label{sec:app}

In this section we show how to apply bias-aware recovery to outlier detection and similarity joins. We will use the sketching and recovery algorithms of bias-aware recovery as black boxes. Let us first assume that the sketching matrix $\Phi$ is a common knowledge known to all the parties in the coordinator model; we will show at the end  of this section how to remove this assumption resource efficiently.

\paragraph{Distributed Outlier Detection}
As briefly mentioned in the introduction, to solve the outlier detection problem in the coordinator model, each site $S^j$ who possesses the vector $\bx^j$ sends $\Phi \bx^j$ to the coordinator; the coordinator then computes $\Phi \bx = \sum_{j \in [\kappa]} \Phi \bx^j$ and uses the recovery algorithm to compute an $\hat{\bx}$ as an approximation of $\bx$.  Here $\Phi$ can be a vertical concatenation of $\Pi(g)$ and $\Psi(h^i, r^i)\ (i \in [d])$ (Algorithm~\ref{alg:l2-sketch}) or a vertical concatenation of $\Upsilon$ and $\Psi(h^i)\ (i \in [d])$ (Algorithm~\ref{alg:l1-sketch}), depending on which error bound (i.e., $\err{1}{}$ or $\err{2}{}$) we desire.   

We spell the algorithm in Algorithm~\ref{alg:outlier}. 

\begin{algorithm2e}[t]
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
\KwIn{$\bx^j \in \mathbb{R}^n$ at each site $S^j$}
\KwOut{$k$ (global) outliers}
\tcc{assume the sketching matrix $\Phi \in \mathbb{R}^{O(k \log n) \times n}$ is common knowledge}
each site $S^j$ computes $\Phi \bx^j$ and sends it to the coordinator\;
the coordinator computes $\Phi \bx = \sum_{j \in [\kappa]} \Phi \bx^j$, and uses Algorithm~\ref{alg:l2-recover} or Algorithm~\ref{alg:l1-recover} to recover $\hat{\bx}$ from $\Phi \bx$\;
the coordinator outputs the $k$ coordinates of $\hat{\bx}$ that deviate the most from the median coordinate of $\hat{\bx}$.
\caption{{\sc Outlier-Detection$(\bx^1, \ldots, \bx^{\kappa})$}}
\label{alg:outlier}
\end{algorithm2e}

By Theorem~\ref{thm:l2} (or Theorem~\ref{thm:l1} which gives the same asymptotic bounds) we have: (1) the sketching time at each site is $O(n \log n)$; (2) the size of the sketch sent by each site is $O(k \log n)$; and (3) the recover time at the coordinator is bounded by $O(\kappa \cdot k \log n + n \log n)$, where the first term counts the time for computing the global sketch $\Phi \bx$.  After obtaining $\hat{\bx}$ which approximates $\bx$ with an additive error $O(k^{-1/p}) \cdot \min_\beta \err{p}(\bx - \beta)$ at each coordinate, the coordinator computes the median of $\hat{\bx}$ and then computes the $k$ outliers.  This post-processing time is $O(n)$.

We summarize the performance of Algorithm~\ref{alg:outlier} in the following theorem.  Let $O$ be the set of top-$k$ indices $i$ that maximize $\abs{x_i - x_M}$, and let $\theta(\bx) = \min\{\abs{x_o - x_M}\ |\ o \in O\}$ (intuitively is the ``threshold'' of becoming a top-$k$ outlier).
\begin{theorem}
There is an algorithm for the outlier detection problem in the coordinator model that computes a set of $k$ outliers $\hat{O}$ so that for any $\hat{o} \in \hat{O}$,
$$\abs{x_{\hat{o}} - x_M} \ge \theta(\bx) - O(k^{-1/p}) \cdot \min_\beta \err{p}(\bx - \beta).$$
The processing time at each site is $O(n \log n)$. The processing time at the coordinator is $O((\kappa k +n)\log n)$.  The communication between each site and the coordinator is $O(k \log n)$. The computation can be done in $1$ round. 
\end{theorem}



\paragraph{Distributed Similarity Joins}
We have briefly mentioned in the introduction how to use bias-aware recovery to solve distributed similarity joins.  Now we give more details.  

Our algorithm for similarity joins in the coordinator model proceeds in $2$ rounds.  In the first round, each site $S^j$ who processes vectors $\bx_{\ell_{j-1}}, \ldots, \bx_{\ell_{j}-1}$ creates $A^j \in \mathbb{R}^{n \times N}$ which is an all-$0$ matrix except the $\ell_{j-1}$-th, $\ldots$, $(\ell_{j}-1)$-th columns being $\bx_{\ell_{j-1}}, \ldots, \bx_{\ell_{j}-1}$. It then computes $\Phi (A^j)^T$ where $\Phi \in \mathbb{R}^{r \times N}$ is the sketching matrix for bias-aware recovery, and sends it to the coordinator. The coordinator then computes $\Phi A^T = \sum_{j \in [\kappa]} \Phi (A^j)^T$.  In the second round, the coordinator sends $\Phi A^T$ to each site. Each site $S^j$ then computes $\Phi A^T \bx_{\ell_{j-1}}, \ldots, \Phi A^T \bx_{\ell_{j}-1}$, uses them to recover the $\ell_{j-1}$-th, $\ldots$, $(\ell_{j}-1)$-th columns of $A^T A$, and then identifies the set $\mathcal{H}^j$ of entries that are at least $\theta$ in those columns.  Finally each $S^j$ sends $\mathcal{H}^j$ to the coordinator, and the coordinator computes and returns $\mathcal{H} = \cup_{j \in [\kappa]} \mathcal{H}^j$.

We spell the algorithm in Algorithm~\ref{alg:join}. 

\begin{algorithm2e}[t]
\DontPrintSemicolon % Some LaTeX compilers require you to use \dontprintsemicolon instead
\KwIn{$S^j$ holds $A^j \in \mathbb{R}^{n \times N}$ consisting of $\bx_{\ell_{j-1}}, \ldots, \bx_{\ell_{j} - 1}\ \in \mathbb{R}^n$ at columns $\ell_{j-1}, \ldots, (\ell_{j}-1)$}
\KwOut{all entries that are at least $\theta$ in $A^T A$ where $A = \sum_{j \in [\kappa]}A^j$}
\tcc{assume the sketching matrix $\Phi \in \mathbb{R}^{O(k\log N) \times N}$ is common knowledge}
each site $S^j$ computes $\Phi (A^j)^T$ and sends it to the coordinator \label{alg:a-1} \;
the coordinator computes $\Phi A^T = \sum_{j \in [\kappa]} \Phi (A^j)^T$, and sends it to each site \label{alg:a-2}\;
each site $S^j$ computes $\Phi A^T \bx_{\ell_{j-1}}, \ldots, \Phi A^T \bx_{\ell_{j}-1}$ and then uses them to recover the $\ell_{j-1}$-th, $\ldots$, $(\ell_{j}-1)$-th columns of $A^T A$ according to Algorithm~\ref{alg:l2-recover} or Algorithm~\ref{alg:l1-recover}. Next, it computes the set $\mathcal{H}^j$ of all entries in these columns that are at least $\theta$, and sends $\mathcal{H}^j$ to the coordinator \label{alg:a-3} \;
the coordinator outputs $\mathcal{H} = \cup_{j \in [\kappa]} \mathcal{H}^j$ \label{alg:a-4}  \; 
\caption{{\sc Similarity Joins$(A^1, \ldots, A^{\kappa})$}}
\label{alg:join}
\end{algorithm2e}

The sketching time at Line~\ref{alg:a-1} of Algorithm~\ref{alg:join} is $O((\ell_{j} - \ell_{j-1}) \cdot n \log N)$, and the sketch size is $O(k \log N)$.  The computation time at Line~\ref{alg:a-2} is $O(\kappa \cdot k\log N \cdot n)$, and the message sent to each site is of size $O(k\log N \cdot n)$.  At Line~\ref{alg:a-3}, the computation time at each site is $O((\ell_{j} - \ell_{j-1}) (k\log N \cdot n + N \log N))$.   

We summarize the performance of Algorithm~\ref{alg:join} in the following theorem.  
%Let $1 = \ell_0 < \ell_1 < \ldots < \ell_{\kappa} = N + 1$; Site $S^j$ holds $(\ell_j - \ell_{j-1})$ vectors $\bx_{\ell_{j-1}}, \ldots, \bx_{\ell_{j}-1} \in \mathbb{R}^n$. 
Let $T^j = \abs{\mathcal{H}^j}\ (j \in [\kappa])$ be the number of outputted pairs that has at least one member in site $S^j$'s input $\{\bx_{\ell_{j-1}}, \ldots, \bx_{\ell_{j}-1}\}$.
%, and let $T = \abs{\mathcal{H}}$ be the total number of output pairs.

\begin{theorem}
There is an algorithm for similarity joins in the coordinator model that outputs all pairs $(u,v)$ with $\bx_u^T \cdot \bx_v \ge \theta$, and no pair with 
$$\bx_u^T \cdot \bx_v \ge \theta - O(k^{-1/p})  \cdot \max_{i \in [N]} \min_{\beta} \err{p}(\by_i - \beta),$$
where $\by_i = A^T \bx_i \in \mathbb{R}^N$.
The processing time at each site $S^j\ (j \in [\kappa])$ is $O((\ell_{j} - \ell_{j-1}) (kn \log N + N \log N))$. The processing time at the coordinator is $O(\kappa k n \log N + \sum_{j \in [\kappa]}T^j)$. The communication between site $S^j$ and the coordinator is $O(k n \log N + T^j)$.\footnote{Note that the size of the input held at site $S^j$ is $(\ell_j - \ell_{j-1}) n$ which is roughly $N n / \kappa$ if the whole input is evenly distributed across the $\kappa$ sites, i.e., $\forall j, \ell_j - \ell_{j-1} \approx N/\kappa$. Therefore our communication cost is sublinear when $T^j$ is small, which is typically the case since we are only interested in those heavily correlated pairs.} The computation can be done in $2$ rounds. 
\end{theorem}


\paragraph{Removing the Common Knowledge $\Phi$ Assumption}
In Algorithm~\ref{alg:outlier} and Algorithm~\ref{alg:join} we assume that $\Phi$ is a common knowledge that is shared among all parties.  We now show how to remove this assumption communication and time efficiently in the coordinator model.

The first observation is that the sampling matrix $\Upsilon$ can be described using $O(\log n)$ words (each of its rows has only one non-zero entry), and thus the coordinator can simply construct one and send it to each site at the beginning of the first round, which costs $O(\log n)$ time and $O(\log n)$ communication with each site.

We next examine sketching matrices $\Pi$'s and $\Psi$'s, which use a set of $O(\log n)$ hash functions $h : [n] \to [s]$ and $r : [n] \to \{1, -1\}$. To make the analysis go through we only need to guarantee that $h$ and $r$ are $4$-wise independent (one only needs to compute the second moments of random variables), and consequently each of them can be described using $O(1)$ words. Thus the coordinator can sample these $O(\log n)$ random hash functions and send them to each site, which costs $O(\log n)$ time and $O(\log n)$ communication with each site.

To sum up, the assumption of using $\Phi$ as a common knowledge in our algorithms can be removed at the cost of spending $O(\log n)$ extra time at the coordinator, and $O(\log n)$ extra communication between each site and the coordinator, and thus will not affect the asymptotic performance of  our algorithms.





==> recovery-speedup.tex <==
\subsection{Recovery Acceleration}
\label{sec:speedup}
In this section we discuss possibly ways to speed up the recovery.  In fact, as shown in \cite{GLPS12}, we can reduce the recovery time to $O(k \log^{O(1)} n)$ using bit-tester matrices, at a cost of increasing the sketch size to $O(k \log^{O(1)} n)$ and the sketching time to $O(n \log^{O(1)} n)$.  This algorithm, however, is a bit complicated to implement for our applications.  

In this section we discuss how to speed up the recovery in the case where all the coordinates of $\bx$ are positive, and our goal is to find those that are larger than a fixed threshold $\theta$ (thus there are at most $\norm{\bx}_1 / \theta$ of them).  

We make use of the tool called {\em dyadic intervals} (used, for example, in \cite{CM04}), which we describe briefly.  We can view dyadic intervals as a binary tree, where the root corresponds to the vector of a single coordinate $\bv_0 = (x_1 + \ldots + x_n)$.  The left child and right child of the root corresponds to the two coordinates in the vector $\bv^1 = (x_1 + \ldots + x_{n/2}, x_{n/2+1} + \ldots + x_{n})$ respectively; and so on. The binary tree has at most $\log n + 1$ levels counting from $0$ (the root).  The $i$-node at the $\ell$-th level of the tree corresponds to the $i$-th coordinate of the vector $\bv^\ell$ whose $j$-th $(j \in [2^\ell])$ coordinate is $x_{(j-1) \cdot n/2^\ell+1} + \cdot + x_{j \cdot n/2^\ell}$.  We construct $\log n$ sketching matrices $\Phi^\ell \in \mathbb{R}^{O(k \log n) \times 2^\ell}$, one for the vector $\bv^\ell$ at each level $\ell \in \{1, \ldots, \log n\}$.  

In the recovery we proceed level by level. We first mark the root {\em red}.  At each level $\ell$, for each red node we recover its corresponding coordinate in $\bv$ using $\Phi^\ell \bx^\ell$; if the coordinate is at least $\theta$ we mark its two child nodes red.  Ignoring the small error at the recovery of each coordinate, at the end of the process we will need to process at most $\min\{\norm{\bx}_1 / \theta \cdot \log n, 2n\}$ nodes, and the time spent on each node is $O(1)$. We therefore can accelerate the recovery procedure in the case when $\theta$ is large, at the cost of increasing the sketching time and sketch size by a factor of $\log n$ (recall that we need to maintain $\log n$ sketches $\Phi^\ell \bv^\ell\ (\ell \in [\log n])$)

